Probabilistic Dalek -- Emulator framework with probabilistic prediction for supernova tomography

Supernova spectral time series can be used to reconstruct a spatially resolved explosion model known as supernova tomography. In addition to an observed spectral time series, a supernova tomography requires a radiative transfer model to perform the inverse problem with uncertainty quantification for a reconstruction. The smallest parametrizations of supernova tomography models are roughly a dozen parameters with a realistic one requiring more than 100. Realistic radiative transfer models require tens of CPU minutes for a single evaluation making the problem computationally intractable with traditional means requiring millions of MCMC samples for such a problem. A new method for accelerating simulations known as surrogate models or emulators using machine learning techniques offers a solution for such problems and a way to understand progenitors/explosions from spectral time series. There exist emulators for the TARDIS supernova radiative transfer code but they only perform well on simplistic low-dimensional models (roughly a dozen parameters) with a small number of applications for knowledge gain in the supernova field. In this work, we present a new emulator for the radiative transfer code TARDIS that not only outperforms existing emulators but also provides uncertainties in its prediction. It offers the foundation for a future active-learning-based machinery that will be able to emulate very high dimensional spaces of hundreds of parameters crucial for unraveling urgent questions in supernovae and related fields.

==> sections/related_work.tex <==
%!TEX root = ../dalek.tex

\section{Related work \label{sec:related_work}}


\subsection{Uncertainty estimation}

Numerous publications extend neural networks to quantify the prediction by uncertainties. Recently popular approaches of Bayesian methods include Monte Carlo (MC) dropout \cite{gal2016dropout} and weight uncertainty \cite{blundell2015weight}. In addition, there are non-Bayesian approaches, for instance, post-hoc calibration by temperature scaling of a validation dataset \cite{guo2017calibration}, and deep ensembles \cite{NIPS2017_9ef2ed4b}. Amongst the classical methods, deep ensembles \cite{NIPS2017_9ef2ed4b} generally perform best in uncertainty estimation \cite{NEURIPS2019_8558cb40}. Methods such as weight uncertainty, MC dropout, and deep ensembles require multiple passes to obtain the uncertainty. For computational efficiency, deterministic methods in a single forward pass \cite{van2020uncertainty, NEURIPS2020_543e8374} are presented. Since our model is a relatively small network which does not take a large amount of computation, we choose the best uncertainty prediction, viz.\ deep ensembles.


